PromptASR for contextualized ASR with controllable style

Prompts are crucial to large language models as they provide context information such as topic or logical relationships. Inspired by this, we propose PromptASR, a framework that integrates prompts in end-to-end automatic speech recognition (E2E ASR) systems to achieve contextualized ASR with controllable style of transcriptions. Specifically, a dedicated text encoder encodes the text prompts and the encodings are injected into the speech encoder by cross-attending the features from two modalities. When using the ground truth text from preceding utterances as content prompt, the proposed system achieves 21.9% and 6.8% relative word error rate reductions on a book reading dataset and an in-house dataset compared to a baseline ASR system. The system can also take word-level biasing lists as prompt to improve recognition accuracy on rare words. An additional style prompt can be given to the text encoder and guide the ASR system to output different styles of transcriptions. The code is available at icefall.

==> text/related_works.tex <==
\section{Related Works}
\label{sec:related}

\subsection{Contextualized ASR}

Depending on the form of the context, most existing contextualized ASR systems falls into the following two categories: word-list context and utterance-level context. The prior one aims at improving the the recognition accuracy on rare words such as contact names. 
~\cite{BrianTCPGen} used a tree-based pointer to boost the posterior of a words in a context list if the prefix matches. ~\cite{CPPBiasing} proposed a neural network-based method to improve rare-word recognition on various E2E ASR architectures, where a text encoder is co-trained with the ASR system to predict if a word/phrase in the context list is present in the utterance. 
Unlike the word list-based context, utterance-level context carries more sophisticated information such as topic and logical relationships. Chang et.al~\cite{SelfAttnBiasing} proposed to inject the embedding of the transcription of previous utterances encoded by a BERT~\cite{BERT} model to the decoder of a neural transducer model and improved the long-form ASR~\cite{longformASR} performance. The word-level embeddings are compressed to a single embedding vector through self-attentive pooling. Li et.al~\cite{llamaPrompt} used LLaMa~\cite{llama} as decoder of the speech encoder to facilitate domain adaptation through text prompts such as topic descriptions.

